A Sketch Is Worth a Thousand Words: Image Retrieval with Text and Sketch

We address the problem of retrieving images with both a sketch and a text query. We present TASK-former (Text And SKetch transformer), an end-to-end trainable model for image retrieval using a text description and a sketch as input. We argue that both input modalities complement each other in a manner that cannot be achieved easily by either one alone. TASK-former follows the late-fusion dual-encoder approach, similar to CLIP, which allows efficient and scalable retrieval since the retrieval set can be indexed independently of the queries. We empirically demonstrate that using an input sketch (even a poorly drawn one) in addition to text considerably increases retrieval recall compared to traditional text-based image retrieval. To evaluate our approach, we collect 5,000 hand-drawn sketches for images in the test set of the COCO dataset. The collected sketches are available a https://janesjanes.github.io/tsbir/.

==> figures/fig_failure.tex <==
\begin{figure*}[t]
  \centering
  \includegraphics[width=0.76\linewidth]{images/limitation_r10.pdf}
   \caption{Two example failure cases.
   The top row in each case shows retrieved images when the model is presented with an input text description (at the top), and a sketch (left).
   For comparison, the bottom row shows retrieved images with only the text description.
   Our model assumes that the input sketch is informative. 
   When the sketch does not accurately represent the target image, this can lead to irrelevant results. 
   We note that for these two examples, the presence of 
   an (inaccurate) input sketch does not enable the model to rank the ground truth image (highlighted with a green border) to be in the top five results.
   }
   \label{fig:limitation} 
\end{figure*}

==> figures/fig_sketch_cap.tex <==
\begin{figure*}[!h]
  \centering
  \includegraphics[height=0.2\textheight]{images/sketch_captioning.pdf}
 \caption{Example of sketch captions generated by our network. 
 While there are some inaccurate details,
 overall the network appears to be able to pick up general ideas of each sketch. 
%  Note that the network tends to start each caption with ``a man'' or ``a woman'' regardless of the content.
}
  \label{fig:sketch_cap}
\end{figure*}

==> sections/conclusion.tex <==
\section{Conclusion}
In this paper, we present \ourmethod; a sketch and text image retrieval system that leverage pre-trained transformer based network from CLIP \cite{clip-radford21a}. 
\label{sec:conclusion}
